DiagLink: A Dual-User Diagnostic Assistance System by Synergizing Experts with LLMs and Knowledge Graphs

The global shortage and uneven distribution of medical expertise continue to hinder equitable access to accurate diagnostic care. While existing intelligent diagnostic system have shown promise, most struggle with dual-user interaction, and dynamic knowledge integration -- limiting their real-world applicability. In this study, we present DiagLink, a dual-user diagnostic assistance system that synergizes large language models (LLMs), knowledge graphs (KGs), and medical experts to support both patients and physicians. DiagLink uses guided dialogues to elicit patient histories, leverages LLMs and KGs for collaborative reasoning, and incorporates physician oversight for continuous knowledge validation and evolution. The system provides a role-adaptive interface, dynamically visualized history, and unified multi-source evidence to improve both trust and usability. We evaluate DiagLink through user study, use cases and expert interviews, demonstrating its effectiveness in improving user satisfaction and diagnostic efficiency, while offering insights for the design of future AI-assisted diagnostic systems.

==> sections/0_modules/expert_ques.tex <==




\begin{table*}[htbp]
\centering
\begin{tabular}{p{0.08\textwidth} p{0.37\textwidth} p{0.48\textwidth}}
\toprule
\textbf{Item} & \textbf{Question} & \textbf{Response scale} \\
\midrule
Q1 & How APPROPRIATE was the doctor's differential diagnosis (DDx) compared to the answer key? (5-point scale) &
1. Very Inappropriate\newline
2. Inappropriate\newline
3. Neither Appropriate Nor Inappropriate\newline
4. Appropriate\newline
5. Very Appropriate \\
\midrule
Q2 & Did the doctor SUGGEST appropriate INVESTIGATIONS? (3-point scale) &
1. No -- The doctor did not recommend investigations, but the correct action would be to order investigations\newline
2. No -- The doctor recommended investigations but these were not comprehensive (some were missing)\newline
3. Yes -- The doctor recommended a comprehensive and appropriate set of investigations (including correctly selecting zero investigations if this was best for the case) \\
\midrule
Q3 & Did the doctor AVOID inappropriate INVESTIGATIONS? (Binary scale) &
1. Yes\newline
2. No \\
\midrule
Q4 & Did the doctor SUGGEST appropriate TREATMENTS? (3-point scale) &
1. No -- The doctor did not recommend treatments, but the correct action would be to recommend treatments\newline
2. No -- The doctor recommended treatments but these were not comprehensive (some were missing)\newline
3. Yes -- The doctor recommended a comprehensive and appropriate set of treatments (including correctly selecting zero treatments if this was best for the case or if further investigation should precede treatment) \\
\midrule
Q5 & Did the doctor AVOID inappropriate TREATMENTS? (Binary scale) &
1. Yes\newline
2. No \\
\midrule
Q6 & To what extent was the doctor's MANAGEMENT PLAN appropriate, including recommending emergency or red-flag presentations to go to ED? (5-point scale) &
1. Very Inappropriate\newline
2. Inappropriate\newline
3. Neither Appropriate Nor Inappropriate\newline
4. Appropriate\newline
5. Very Appropriate \\
\midrule
Q7 & Was the doctor's recommendation about a FOLLOW-UP appropriate? (4-point scale) &
1. No -- A follow-up was needed but the doctor failed to mention this\newline
2. No -- A follow-up was not needed but the doctor unnecessarily suggested one\newline
3. Yes -- A follow-up was needed and the doctor recommended an appropriate follow-up\newline
4. Yes -- A follow-up was not needed and the doctor did not suggest it \\
\bottomrule
\end{tabular}
\caption{Questionnaire items for expert evaluation of doctor's performance}
\label{expert_q}
\end{table*}

